Global-Local Forward Models within Bayesian Inversion for Large Strain Fracturing in Porous Media

In this work, Bayesian inversion with global-local forwards models is used to identify the parameters based on hydraulic fractures in porous media. It is well-known that using Bayesian inversion to identify material parameters is computationally expensive. Although each sampling may take more than one hour, thousands of samples are required to capture the target density. Thus, instead of using fine-scale high-fidelity simulations, we use a non-intrusive global-local (GL) approach for the forward model. We further extend prior work to a large deformation setting based on the Neo-Hookean strain energy function. The resulting framework is described in detail and substantiated with some numerical tests.

==> DD27_MSBI 2/commands.tex <==
% Operators
\newcommand{\curl}[1]{\text{curl}\left(#1\right)}
\newcommand{\dd}{\mathsf{d}}

% Spaces:
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\Hcurl}[1]{\mathbf{H}\left(\text{curl, }#1\right)}

% Traces:
\newcommand{\trace}[1]{\gamma^T\left(#1\right)}
\newcommand{\curltrace}[1]{\gamma^t\left(#1\right)}

\newcommand{\tracei}[2]{\gamma^T_#1\left(#2\right)}
\newcommand{\curltracei}[2]{\gamma^t_#1\left(#2\right)}

\newcommand{\skin}[1]{\textcolor{blue}{#1}}
\definecolor{lightblue}{RGB}{0, 142, 255}
\newcommand{\skremark}[1]{\textcolor{lightblue}{SK: #1}}
\definecolor{sblue}{RGB}{0, 10, 255}
\newcommand{\SB}[1]{\textcolor{sblue}{SB: #1}}


